Antelope: Potent and Concealed Jailbreak Attack Strategy

Due to the remarkable generative potential of diffusion-based models, numerous researches have investigated jailbreak attacks targeting these frameworks. A particularly concerning threat within image models is the generation of Not-Safe-for-Work (NSFW) content. Despite the implementation of security filters, numerous efforts continue to explore ways to circumvent these safeguards. Current attack methodologies primarily encompass adversarial prompt engineering or concept obfuscation, yet they frequently suffer from slow search efficiency, conspicuous attack characteristics and poor alignment with targets. To overcome these challenges, we propose Antelope, a more robust and covert jailbreak attack strategy designed to expose security vulnerabilities inherent in generative models. Specifically, Antelope leverages the confusion of sensitive concepts with similar ones, facilitates searches in the semantically adjacent space of these related concepts and aligns them with the target imagery, thereby generating sensitive images that are consistent with the target and capable of evading detection. Besides, we successfully exploit the transferability of model-based attacks to penetrate online black-box services. Experimental evaluations demonstrate that Antelope outperforms existing baselines across multiple defensive mechanisms, underscoring its efficacy and versatility.

==> sec/reference.tex <==
\section{Reference}
\textbf{SneakyPrompt} \cite{sneakyprompt}:  Intuitive approaches will be brute force, beam, or greedy searches, but they are often cost-ineffective, e.g., incurring many queries to the target text to-image model. Adversarial examples are carefully crafted inputs to confuse a learning model for an incorrect decision, e.g., wrong classification results.  There are generally two directions on adversarial text examples. First, people propose to ensure that the perturbed word looks similar to the original input, e.g., “nice” vs “n1ce”. Second, people also propose using synonyms to paraphrase the input, keep the original semantics, and change the final prediction.

\textbf{PRISM} \cite{AutomatedBP}: The key difference between PRISM and prior methods is that PRISM updates the entire sampling distribution of prompts, whereas prior works  directly update the tokens of a single prompt or the embedding of the prompt. Effective prompts for T2I models are often not
 grammatically correct sentences but rather collection of phrases that de
scribe the details about the image, which generic captioning models are
 not trained to generate. 

\textbf{ConceptPrune} \cite{conceptprune}: We show that neurons in LDMs often specialise to specific concepts, and that pruning these neurons can be used to
permanently eliminate undesired concepts from image generation.

\textbf{JPA} \cite{jpa}:  Our key insight is to search unique extra tokens for a given NSFW prompt to jailbreak the safety checkers while still preserving the semantics of the prompt and the follow-up generated NSFW images. We first use a
 simple concatenation method to combine extra learnable tokens and NSFW prompts and use cosine similarity metric to
 keep the concatenated prompts semantically similar to the rendered embedding. At the same time search within the vocabulary range of the token space to find the extra learnable tokens.
JPA finds adversarial prompts in the sensitive region of the text space by
adding learnable tokens to each prompt.  For nudity and violence, we find these Unicode symbols often appear in adversarial prompts, and the emojis of
 them may have dangerous meanings.
 We believe that the semantic attributes contained in such soft embeddings,
 which can be added or subtracted, stem from the initial semantic alignment capability in the pre-trained text space.
\textbf{ The two concepts tested in our experiment have their own ground truth datasets, each containing
 1000 images generated by NSFW-142 and NSFW-90 respectively.}

\textbf{Comprehensive} \cite{comprehensive} : To provide a structured overview of the strategies
 utilized to compromise LLMs, we categorize current attack techniques into three categories, reflecting their fundamental traits. The first category, Generative Techniques, includes attacks that are dynamically produced, eschewing predetermined plans. The second category, Template Techniques, comprises attacks conducted via pre-defined templates or modifications in the generation settings. The last category, Training Gaps Techniques, focuses on exploiting weaknesses due to insufficient safeguards in safe training practices, such as
 RLHF. We further conduct thorough examination on the existing defense mechanisms, classifying them into
 three categories based on their operational principles: Self-Processing Defenses, which rely exclusively on the LLM’s own capabilities; Additional
 Helper Defenses, which require the support of additional algorithms or auxiliary LLMs for verification purposes; and Input Permutation Defenses, which manipulate the input prompt and veritfy with the target LLMs mutliple times to detect and counteract malicious requests aimed at exploiting gradient-based vulnerabilities.

 \textbf{AutoDefense} \cite{autodefense}: Existing defense methods against LLM
 jailbreak attacks can be divided into prompt-based
 and response-based defenses.  Prompt-based de
fenses like System-Mode Self-Reminder  use a specially-designed prompt to remind LLM not to generate harmful or misleading content. In contrast, response-based defenses first feed an input prompt into an LLM to generate a response, and then evaluate whether the response is harmful.

\textbf{BackdoorAlign} \cite{backdooralign}:  Our method constructs prefixed safety examples with a secret prompt, acting as a “backdoor trigger,” that is strategically prefixed to the safety examples and remains unseen by users. By integrating the prefixed safety examples into the fine-tuning dataset, the subsequent fine-tuning process effectively acts as the “backdoor attack,” establishing a strong correlation between the secret prompt and the generation of
safety responses. 

\textbf{RING-A-BELL} \cite{ringabell}: Detection-based methods aim to remove inappropriate content by
 filtering it through safety checkers while removal-based methods tries to steer the model away from
 those contents by actively guiding in inference phase or fine-tuning the model parameters.

 \textbf{MMP-Attack} \cite{mmp}:  the prompts are embedded chaotically in the text feature space, while in the image feature space they are clustered according to their subjects. Our approach optimizes a
 suffix appended to the original prompt, aiming to effectively
 facilitates the generation of a desired target object by remov
ing the original object, thus addressing the most challenging
 scenario. In the text feature
space, prompts with different subjects but originating from the same template can be embedded close together.

\textbf{PGJ} \cite{PGJ}: The idea comes from the observation we term perceptual confusion: due to perceptual
similarity, people may become confused about the objects or behaviors depicted in an image (e.g., flour in an image may look like heroin). Thus we propose finding a safe phrase (comprising one or more words) that can induce perceptual confusion with the target unsafe word to use as a
 substitution. To be specific, we propose to find the safe substitution
 phrase according to the PSTSI principle, i.e., the safe
 substitution phrase and target unsafe word should be similar in human perception and inconsistent in text semantics. Currently, more and more works have put emphasis on exploring the opened avenues for
 potential misuse of T2I models, particularly in generating
 inappropriate or NSFW content via adversarial attack. SneakyPrompt  exploits reinforcement learning to
 replace the words in the prompt for bypassing safety filters
 in T2I generative models. SurrogatePrompt  proposes
 a pipeline that contains three modules to generate NSFW
 images on T2I models such as Midjourney and DALL·E 2.
 DACA  breaks down unethical prompts into multiple benign descriptions of individual image elements and makes
 word substitutions for each element. MMA-Diffusion is
 a multimodal attack framework that designs attacks on both
 text and image modalities. UPAM is a unified framework
 that employs gradient-based optimization, sphere-probing
 learning, and semantic-enhancing learning to attack the T2I
 model. JPA  using learnable tokens to create adversarial
 prompts that evade detection while preserving the semantic
 integrity of the original NSFW content.

 \textbf{QF-Attack} \cite{QFattack}: we empirically show that only a five-character perturbation to the text prompt is able to cause the significant content shift of synthesized images using Stable Diffusion. 


 \textbf{MMA-Diffusion} \cite{mma}:  MultiModal Attack on Diffusion Models. Inspired by gradient-driven optimization methods from the NLP domain like LLM-attack [42], FGPM [38], TextGrad [11], and prompt learning techniques [36], we harness token-level gradients to guide the optimization process. To search substitutional tokens, we utilize a greedy search strategy. To find such a free-style adversarial prompt, we introduce the search method based on gradient optimization.  w Given that the image is prone to NSFW contents induced by malicious prompts, we aim to evade the post-hoc safety checker through the adversarial
 attack. We employ the Attack Success Rate
 out of N syntheses(ASR-N) as our evaluatio nmetric. To
 compute ASR-N, wecommand T2I to generate N images
 for each prompt. If any of these images exhibit NSFW content and bypass our simple prompt filter, the attack is considered successful. UnlearnDiff primarily examines concept-erased dif
fusion models [7, 15, 30, 34] and does not extend to other
 defense strategies. Conversely, Ring-A-Bell [37] explores
 inducing T2I models to generate NSFW concepts but lacks
 precision in controlling the details of the synthesis. 


  \textbf{UnlearnDiffAtk} \cite{unlearndiffatk}: In text-to-image generation, various inputs such as text prompts, random seed values, and guidance scales can be altered to generate diverse images [7]. Hence, we assess the robustness of unlearned DMs using
 their original prompt, random seed, and guidance scale configurations for each
 unlearning instance.  When facing inappropriate test prompts, we will dissect the
 attack success rate (ASR) into two categories: (1) the pre-attack success rate
 (pre-ASR), and (2) the post-attack success rate (post-ASR). 

 \textbf{RT-Attack} \cite{RTattack} Unlike existing methods, such as the technique used in MMA-Diffusion (Yang et al. 2024c), which requires perturbations in both text and image modalities to bypass post-hoc image checkers, our method focuses solely on perturbing the text input. Ring-A-Bell explores techniques for inducing T2I models to generate NSFW content but lacks precise control over the specifics of the synthesis process.In contrast, UnlearnDiff focuses on concept-erased diffusion models, yet does not investigate other defensive strategies.

